A Large Scale Investigation of Obfuscation Use in Google Play

Android applications are frequently plagiarized or repackaged, and software obfuscation is a recommended protection against these practices. However, there is very little data on the overall rates of app obfuscation, the techniques used, or factors that lead to developers to choose to obfuscate their apps. In this paper, we present the first comprehensive analysis of the use of and challenges to software obfuscation in Android applications. We analyzed 1.7 million free Android apps from Google Play to detect various obfuscation techniques, finding that only 24.92% of apps are obfuscated by the developer. To better understand this rate of obfuscation, we surveyed 308 Google Play developers about their experiences and attitudes about obfuscation. We found that while developers feel that apps in general are at risk of plagiarism, they do not fear theft of their own apps. Developers also self-report difficulties applying obfuscation for their own apps. To better understand this, we conducted a follow-up study where the vast majority of 70 participants failed to obfuscate a realistic sample app even while many mistakenly believed they had been successful. Our findings show that more work is needed to make obfuscation tools more usable, to educate developers on the risk of their apps being reverse engineered, their intellectual property stolen, their apps being repackaged and redistributed as malware and to improve the health of the overall Android ecosystem.

==> includes/evaluate_apks.tex <==
\begin{lstlisting}[%
    basicstyle=\footnotesize,
    frame=none,
    numbers=right,
    numbersep=0pt,
    numberstyle=\tiny\color{gray},
    breaklines
]
a2dp.Vol_126_src-release.apk,
app.varlorg.unote_7_src-release.apk,
at.bitfire.gfxtablet_5_src.apk,
at.linuxtage.companion_9_src.apk,
au.com.wallaceit.reddinator_52_src.apk,
axp.tool.apkextractor_1_src.apk,
be.brunoparmentier.dnssetter_3_src.apk,
be.digitalia.fosdem_700136_src.apk,
be.quentinloos.manille_2_src.apk,
be.uhasselt.privacypolice_9_src.apk,
biz.codefuture.svgviewer_8_src.apk,
br.usp.ime.retrobreaker_5_src.apk,
ca.rmen.android.frenchcalender_192_src.apk,
ca.rmen.android.networkmonitor_12804_src.apk,
ca.rmen.android.poetassistant_182_src.apk,
ca.rmen.android.scrumchatter_10302_src.apk,
ca.rmen.nounours_340_src.apk,
cat.mvmike.minimalcalendarwidget_1_src.apk,
ch.blinkenlights.android.vanilla_10430_src.apk,
ch.corten.aha.worldclock_44_src.apk,
ch.ihdg.calendarcolor_4_src.apk,
click.dummer.textthing_18_src.apk,
co.loubo.icicle_4_src.apk,
com.aaronjwood.portauthority_35_src.apk,
com.actisec.clipcaster_48_src.apk,
com.adam.aslfms_40_src.apk,
com.agnibho.android.solarcompass_1_src.apk,
com.akop.bach_120_src.apk,
com.alexkang.bluechat_2_src.apk,
com.alexkang.loopboard_19_src.apk,
com.amabyte.vtucslabmanual_1_src.apk,
com.anddevw.getchromium_20160614_src.apk,
com.app.missednotificationsreminder_1801010500_src.tar.gz-v14-release-v1.1.5.apk,
com.axelby.podax_63_src.tar.gz-release.apk,
com.blanyal.remindly_2_src.apk,
com.bleyl.recurrence_23_src.apk,
com.briankhuu.nfcmessageboard_13_src.apk,
com.bytestemplar.tonedef_16_src.apk,
com.casimirlab.simpleDeadlines_19_src.apk,
com.catchingnow.tinyclipboardmanager_57_src.apk,
com.claha.showtimeremote_2_src.apk,
com.cr5315.cfdc_27_src.apk,
com.danielkim.soundrecorder_5_src.apk,
com.daviancorp.android.mh4udatabase_9_src.apk,
com.developfreedom.wordpowermadeeasy_12_src.apk,
com.dimtion.shaarlier_20_src.apk,
com.dnielfe.manager_67_src.apk,
com.dnielfe.manager_67_src-release.apk,
com.doomy.overflow_4_src.apk,
com.doomy.torch_11_src.apk,
com.doomy.torch_11_src-release.apk,
com.ds.avare_230_src.apk,
com.easwareapps.micopi_32_src.apk,
com.easwareapps.quoter_3_src.apk,
com.easwareapps.quoter_3_src-release.apk,
com.easwareapps.transparentwidget_2_src.apk,
com.ebaschiera.triplecamel_5_src.apk,
com.ecuamobi.deckwallet_100_src.apk,
com.eibriel.reddot_3_src-release.apk,
com.enrico.filemanager_4_src-release.apk,
com.gelakinetic.mtgfam_43_src-release.apk,
com.gunshippenguin.openflood_9_src-release.apk,
com.jorgecastillo.kanadrill_28_src-release.apk,
com.jparkie.givesmehope_6_src-release.apk,
com.markusborg.test_17_src-release.apk,
com.moonpi.swiftnotes_9_src-release.apk,
com.morlunk.mumbleclient_73_src-release.apk,
com.mridang.speedo_2_src-release.apk,
com.omegavesko.sutransplus_1_src-release.apk,
com.samsung.srpol_9_src-release.apk,
com.serwylo.lexica_904_src-release.apk,
com.simplemobiletools.applauncher_4_src-release.apk,
com.simplemobiletools.calendar_17_src-release.apk,
com.simplemobiletools.draw_9_src-release.apk,
com.simplemobiletools.notes_9_src-release.apk,
com.tjm.stripepaper_2_src-release.apk,
com.vlille.checker_611_src-release.apk,
com.workingagenda.devinettes_1_src-release.apk,
cz.eutopia.snooperstopper_4_src-release.apk,
de.hoffmannsgimmickstaupunkt_16_src.tar.gz-release.apk,
de.naturalnet.zahnarztgeraeusche_1_src-release.apk,
de.onyxbits.droidentify_3_src.tar.gz-release.apk,
ee.ioc.phon.android.speak_1206_src-release.apk,
free.rm.skytube.oss_1_src-release.apk,
fr.tvbarthel.apps.cameracolorpicker_7_src-release.apk,
indrora.atomic_21_src-release.apk,
IthakaBoardGame-release.apk,
me.anuraag.grader_3_src-release.apk,
min-cal-widget-release.apk,
net.sf.times_37_src-release.apk,
networkmonitor-1.28.4-foss-release.apk,
nwswidget-release.apk,
org.androidpn.client_20160415_src-release.apk,
org.legtux.m_316k.fortune_1_src-release.apk,
org.transdroid.lite_227_src-release.apk,
org.transdroid.search_28_src-release.apk,
org.xphnx.ameixa_37_src-release.apk,
sony.hidden.servicemenu_2_src-release.apk,
uk.co.ashtonbrsc.android.intentintercept_224_src-release.apk,
yellr.net.yellr_android_1008_src-release.apk
\end{lstlisting}

==> includes/proguard_reasons.tex <==
\begin{table}
	\centering
	\begin{tabular}{lccc}
		\toprule
		Benefit                             & Dev       & User      & Ecos \\
		\midrule
		Repackaging Protection              & \yes{}    & \yes{}    & \yes{}    \\
		Intellectual Property Protection    & \yes{}    & \kinda{}  & \kinda{}  \\
		Ad-revenue Protection               & \yes{}    & \no{}     & \kinda{}  \\
	    \midrule
	    Performance Optimization            & \yes{}    & \yes{}    & \kinda{}  \\
		{APK} Size Reduction                & \yes{}    & \yes{}    & \yes{}    \\
		\bottomrule
	\end{tabular}
	\caption[Benefits of {ProGuard} for app developers, app users and the entire ecosystem.]{Benefits of {ProGuard} for app developers, app users and the entire ecosystem. Benefits are marked as direct benefits (\yes{}) partial benefits (\kinda{}), and no benefits (\no{}).}\label{tbl:proguard_reasons}
\end{table}

==> sections/benefits.tex <==
Obfuscation provides a defense against several undesired activities. 
First, it protects design secrets from being made public. In situations where algorithms or trade secrets are embedded in application code, obfuscation makes these secrets more difficult to acquire. 
More importantly, software obfuscation prevents code theft and reuse. 
Many developers (including our survey participants) primarily think of this problem as one of a
legitimate competitor stealing portions of code to simplify their own
development. This is a rare and unlikely practice.
A far more common practice is wholesale app theft --- known as
repackaging --- where an adversary copies the entire app. This can
be done to insert malicious code or to profit from an
existing app's popularity by repackaging it and releasing the app onto third party
markets (perhaps at a lower price) with different advertising
libraries that pay the repackager~\cite{whatsapp2017}.

The practice of repackaging is epidemic,
and represents a threat to the entire ecosystem. Zhou et al.\ found that 86\% of malware samples they collected were repackaged versions of benign applications~\cite{zhou2012a}, and in a related project found that up to 13\% of entire third party markets consist of plagiarized, repackaged apps~\cite{zhou2012b,zhou2013}. Other measurements have shown that apps are repackaged by the thousands~\cite{viennot2014,crussell2015}, and in fact one of our participants was a victim of app repackaging on multiple occasions.
The consequence of this is that end users are regularly
threatened by malicious code, and app developers risk losing revenue
that is being stolen by adversaries in advertising fraud. Moreover,
by infecting devices or cheating developers
the practice of app repackaging threatens the popularity of the
platform for both end users and developers alike.
Software obfuscation provides a practical solution to this problem, and while  software obfuscation does not entirely eliminate the threats of IP theft or repackaging, it raises the costs for attackers. 

We note that the benefits of obfuscation certainly depend on the efficacy of the obfuscation applied.
In this paper, we focus on {ProGuard}~\footnote{Though not to the exclusion of
other obfuscations tools. See section \ref{subsec:other_tools} for details.}. Though {ProGuard} is not
as technically sophisticated as other tools, we find that it is the most
commonly used tool in Android applications. We expect this is due to the fact that {ProGuard} is freely available to developers and built in to Android Studio.
We find that only 0.22\% of apps use what is likely a non-ProGuard-related obfuscation tool. 

The ultimate effectiveness of software obfuscation is in many ways an open question; there is much anecdotal evidence about the effectiveness of various obfuscations, but little rigorous empirical evidence of this. What little literature exists finds that software obfuscation can significantly increase the costs of both automated and manual analyses~\cite{ceccato2009,ceccato2014,schrittwieser2016}. We note that while the question is beyond the scope of this work, more
evidence is needed to characterize the effectiveness of software
obfuscation, especially for mobile applications, as well as the effectiveness of obfuscation on preventing repackaging. As this paper is the first step in analyzing obfuscation of \emph{legitimate software} in the Android ecosystem, we hope that the techniques we develop in this work will facilitate such analyses in future work.
